Improving Object Detection with Inverted Attention

Improving object detectors against occlusion, blur and noise is a critical step to deploy detectors in real applications. Since it is not possible to exhaust all image defects through data collection, many researchers seek to generate hard samples in training. The generated hard samples are either images or feature maps with coarse patches dropped out in the spatial dimensions. Significant overheads are required in training the extra hard samples and/or estimating drop-out patches using extra network branches. In this paper, we improve object detectors using a highly efficient and fine-grain mechanism called Inverted Attention (IA). Different from the original detector network that only focuses on the dominant part of objects, the detector network with IA iteratively inverts attention on feature maps and puts more attention on complementary object parts, feature channels and even context. Our approach (1) operates along both the spatial and channels dimensions of the feature maps; (2) requires no extra training on hard samples, no extra network parameters for attention estimation, and no testing overheads. Experiments show that our approach consistently improved both two-stage and single-stage detectors on benchmark databases.

==> tex/method.tex <==
\section{Method}
Our proposed framework includes three part. First, we train a detection model as teacher network. Then we we use some attention mechanism to extract most discriminative region from teacher network. Finally, we utilize generated attention maps as guidance to dropout critical spatial and channel part in feature maps when training student network. 

\subsection{Baseline Model}
Our model is built based on Fast-RCNN framework. Given an input image, the convolutional network of the Fast-RCNN takes the whole image as an input and produces convolutional feature maps as the output. Given the feature map and pre-computed region proposal candidates, The RoI-pooling layer crops and resizes to generate a fixed size feature vector for each object proposal. These feature vectors are then passed through fully connected layers to predict the probabilities for each object class and bounding box coordinates.

\subsection{Attention Mechanism}
We consider two types of attention maps: gradient-based and activation-based attention.

\subsubsection{gradient-based attention}

